Validated Asynchronous Byzantine Agreement with Optimal Resilience and Asymptotically Optimal Time and Word Communication

We provide a new protocol for Validated Asynchronous Byzantine Agreement. Validated (multi-valued) Asynchronous Byzantine Agreement is a key building block in constructing Atomic Broadcast and fault-tolerant state machine replication in the asynchronous setting. Our protocol can withstand the optimal number $f<n/3$ of Byzantine failures and reaches agreement in the asymptotically optimal expected $O(1)$ running time. Honest parties in our protocol send only an expected $O(n^2)$ messages where each message contains a value and a constant number of signatures. Hence our total expected communication is $O(n^2)$ words. The best previous result of Cachin et al. from 2001 solves Validated Byzantine Agreement with optimal resilience and $O(1)$ expected time but with $O(n^3)$ expected word communication. Our work addresses an open question of Cachin et al. from 2001 and improves the expected word communication from $O(n^3)$ to the asymptotically optimal $O(n^2)$.

==> related.tex <==
\section{Related Work}
\label{sec:related}

==> validity.tex <==
\subsection{The power of validity}
\label{sub:validity}



In this section we compare between of the external and weak validity
properties.
Although they are incomparable, we believe that (1) external validity
is more practical for blockchain systems, and (2) agreement with weak
validity is in some sense an easier problem as we now explain. 

\ldots\ldots\ldots\ldots

Quote rynal's paper when talk about k-set agreement. Impossible for
our validity even in crash model.
Then, explain from practical point of view.

With weaker validity, a deterministic reduction to binary agreement is
possible, but it is impossible with stronger validity. 

Talk about better of both worlds.




%  with external validation.
% The classical validity condition for Byzantine
% agreement~\cite{dolev1983authenticated, cristian1986atomic, algorand,
% Raynalmultivalued, Julian} is the follows:
% 
% 
% \begin{definition}[Classical validity]
% 
% If all honest parties propose $v$, then any honest party that
% terminates decides $v$.
% 
% \end{definition}

We refer to Byzantine agreement with the cassical validity
condition as \emph{classical Byzantine agreement}, or \emph{CBA}, and to the
variant due to Cachin el al.~\cite{..} as \emph{practical Byzantine agreement}, or
\emph{PBA}.
In CBA, if honest parties propose different values, the decision may be
any value.
For example, in~\cite{Raynalmultivalued,algorand,Julian}, parties may
agree on an a priori known default value $\bot$, which is basically
the same as to decide not to decide.

\DM{omitted, I don't think we can quote the book yet; we could quote Cachin
(with permission) as "private communication", but not sure it is needed.}
%From a practical point of view, CBA is not strong
%enough - here is a quote from a recent book dedicated to Lamport's
%work~\cite{lamport-book}:
%
%\begin{quote}
%“validity in Byzantine agreement may not be useful for
%practice applications since it says nothing about  the situation
%where the correct processes start with diverging inputs”
%\end{quote}
%

If Byzantine agreement is used for 
Byzantine state machine replication, then CBA does
not guarantee progress unless all honest parties propose the same value. The
solution is often to employ a leader and wait the maximal network delay for the
leader proposal, e.g., Algorand~\cite{algorand}, Dfinity
Consensus~\cite{Dfinity} and others.

In contrast, solving PBA allows us to implement Byzantine replication without reying on
synchrony. In each round, there is constant probability of success, hence in
expected $O(1)$ rounds progress is made.

